Pixel to Binary Embedding Towards Robustness for CNNs

There are several problems with the robustness of Convolutional Neural Networks (CNNs). For example, the prediction of CNNs can be changed by adding a small magnitude of noise to an input, and the performances of CNNs are degraded when the distribution of input is shifted by a transformation never seen during training (e.g., the blur effect). There are approaches to replace pixel values with binary embeddings to tackle the problem of adversarial perturbations, which successfully improve robustness. In this work, we propose Pixel to Binary Embedding (P2BE) to improve the robustness of CNNs. P2BE is a learnable binary embedding method as opposed to previous hand-coded binary embedding methods. P2BE outperforms other binary embedding methods in robustness against adversarial perturbations and visual corruptions that are not shown during training.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> files/analysis_smooth.tex <==
\begin{figure*}[tbp]
\centering
\begin{subfigure}{0.325\textwidth}
  \includegraphics[width=\linewidth]{figures/p2be.pdf}
  \caption{One-hot}
\end{subfigure}
\begin{subfigure}{0.325\textwidth}
  \includegraphics[width=\linewidth]{figures/p2be_0.pdf}
  \caption{Thermometer}
\end{subfigure}
\begin{subfigure}{0.325\textwidth}
  \includegraphics[width=\linewidth]{figures/p2be_em1.pdf}
  \caption{Random}
\end{subfigure}


\caption{The cosine similarity of binary embeddings. The vertical and horizontal axis represents that the indices $i, j \in [0,...,255]$ corresponding to the magnitude for each RGB value. In table, the cell at the coordinate $(i,j)$ represents the cosine similarity between binary embeddings $e_i$ and $e_j$. The black and white colors indicate that the cosine similarities are 1.0 and 0.0, respectively. Figure (c) is the binary embedding generated by the normal distribution with mean 0 and variance 1. The dimension of binary embeddings $M$ is 64. C-10, C-100 and IN-1k represent CIFAR-10, CIFAR-100 and ImageNet-1k datasets, respectively. WRN, R50, DN and RN represent WideResNet, ResNet50, DenseNet and ResNext, respectively.}
\label{fig:cos}
\end{figure*}

==> files/checklists.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%%The checklist follows the references.  Please
%%read the checklist guidelines carefully for information on how to answer these
%%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%%justification to your answer}, either by referencing the appropriate section of
%%your paper or providing a brief inline description.  For example:
%%\begin{itemize}
%%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%%  \item Did you include the license to the code and datasets? \answerNA{}
%%\end{itemize}
%%Please do not modify the questions and only use the provided macros for your
%%answers.  Note that the Checklist section does not count towards the page
%%limit.  In your paper, please delete this instructions block and only keep the
%%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Lines 193-195, 208-211 and 219-223}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> files/experiments_c_detection.tex <==
%%%%%%%%%%   COCO-C
\paragraph{Implementation Details.}
#TBD
\paragraph{Result.}
#TBD
\begin{table}[htbp]
  \centering
  \caption{The mean performance
under corruption (mPC) on COCO-C dataset.}
  \label{tab:cifar_adv}
  \vspace{0.2cm}
  \begin{tabular}{c|c}
  \hline\noalign{\smallskip}
  & mPC [AP] \\ \hline\noalign{\smallskip}
RGB &  18.1\\
One-hot & 19.3\\
Thermometer & 18.8\\
P2BE (ours) & 19.1\\
  \hline
  \end{tabular}
\end{table}

%%%%%%%%%%   COCO-C
\paragraph{Implementation Details.}
#TBD
\paragraph{Result.}
#TBD
\begin{table}[htbp]
  \centering
  \caption{The mean performance
under corruption (mPC) on COCO-C dataset.}
  \label{tab:cifar_adv}
  \vspace{0.2cm}
  \begin{tabular}{c|c}
  \hline\noalign{\smallskip}
  & Test error \% \\ \hline\noalign{\smallskip}
augmix &  35.2 (22.2)\\
genmix w/ intended implementation& 34.5 (21.8)\\
genmix w/ wrong implementation& 33.5 (22.1)\\

  \hline
  \end{tabular}
\end{table}

